Molecule Design by Latent Prompt Transformer

This work explores the challenging problem of molecule design by framing it as a conditional generative modeling task, where target biological properties or desired chemical constraints serve as conditioning variables. We propose the Latent Prompt Transformer (LPT), a novel generative model comprising three components: (1) a latent vector with a learnable prior distribution modeled by a neural transformation of Gaussian white noise; (2) a molecule generation model based on a causal Transformer, which uses the latent vector as a prompt; and (3) a property prediction model that predicts a molecule's target properties and/or constraint values using the latent prompt. LPT can be learned by maximum likelihood estimation on molecule-property pairs. During property optimization, the latent prompt is inferred from target properties and constraints through posterior sampling and then used to guide the autoregressive molecule generation. After initial training on existing molecules and their properties, we adopt an online learning algorithm to progressively shift the model distribution towards regions that support desired target properties. Experiments demonstrate that LPT not only effectively discovers useful molecules across single-objective, multi-objective, and structure-constrained optimization tasks, but also exhibits strong sample efficiency.

==> scripts/optimization.tex <==
\begin{figure}[H]
\centering
\small
\begin{tikzpicture}[block/.style={rectangle, draw, fill=black!5, minimum width=3cm, minimum height=0.6cm, align=center, rounded corners},
    arrow/.style={->,>=stealth},
    bigbox/.style={draw, thick, rounded corners, inner sep=5pt, dashed}]

\node [block] (generate) {\textbf{Latent Space Sampling}\\$\mathcal{P}^t=\{z^t_i,x^t_i, y^t_i\}_{i=1}^m$\\where $z^t\sim p(z|y=y^{t-1}+\Delta_y)$;\\ $x^t\sim p(x|z=z^t)$};
\node [block, below=of generate, yshift=-0.5cm] (verify) {\textbf{Data Space Selection}\\$\mathcal{D}^{t}=\mathrm{Select}(\{z_i^t,x_i^t,\check{y}_i^t\}_{i=1}^m\cup \mathcal{D}^{t-1})$};
\node [block, left=1.5cm of $(generate)!0.5!(verify)$] (update) { \textbf{Improve LPT}\\$\theta_{t}=$\cref{algo:learning}$(\theta_{t-1}, \mathcal{D}_{t})$};
% \path
% (generate) edge[right]      node{\small $y=o(x)$}          (verify);
% Draw edges
\draw [arrow] (generate) -- (verify) node[midway, right, align=left] {Relabeling \\ $\check{y}^t = o(x^t)$};
\draw [arrow] (verify) -| (update);
\draw [arrow] (update) |- (generate);

\end{tikzpicture}
\caption{Graphical illustration of Dual-Space Optimization (DSO) with LPT at the shifting iteration $t$. The plot of distribution shifting over iterations can be found in~\cref{fig:shift_illustrate}}.
\label{fig:dso}
\vskip -0.15in
\end{figure}

After learning the joint distributions of molecules and properties $p_\theta(x,y)$, our objective is to generate a synthetic dataset of molecules with maximal values of specific target properties, as defined by oracle functions $o(x)$. 
%\begin{align}
%    x^*=\argmax_x \E_{p_\theta(x,y)}[o(x)],
%\end{align} 
%where $y^*$ represents the target property or constraint of interest. 
Following previous studies on molecule design, we assume access to the oracle functions via software such as RDKit~\citep{landrum2013rdkit} and AutoDock-GPU~\citep{santos2021accelerating}. While acknowledging the critical role of these tools in providing accurate property evaluations for molecules, our paper focuses primarily on the optimization process, not the designing of the oracle function. 

In optimization cases where the target value $y^*$ may not be supported within the learned distribution $p_\theta(x,y)$, we introduce an iterative online optimization method. This process is initialized with a pretrained distribution $p_\theta(x,y)$ and gradually shifts the distribution over $T$ iterations. 

Each iteration involves a dual-space sampling strategy: \textit{Latent Space Sampling} for generating proposals and \textit{Data Space Selection} for refinement of the synthetic dataset by the oracle function and \textit{Improve LPT} based on the refined dataset, termed as Dual-Space Optimization (DSO). We provide an overview and a demonstration of the DSO in \cref{fig:dso} and \cref{fig:shift_illustrate}.

In this iterative framework, the optimization problem at iteration $t$ is as follows: Given the trained model at the previous time step $p_{\theta_{t-1}}(z,x,y)$ and the shifting dataset $\mathcal{D}^{t-1}=\{z_i^{t-1},x_i^{t-1},y_i^{t-1}\}_{i=1}^n$, we aim to sample proposals $\mathcal{P}^t=\{z_i^{t},x_i^{t},y_i^{t}\}$ to create an improved synthetic dataset $\mathcal{D}^{t}$. This new dataset is designed to exhibit improved desired properties over $\mathcal{D}^{t-1}$, allowing fitting and refining our model progressively. The initial dataset $\mathcal{D}^0$ is composed of the top-$n$ samples with desired values from the offline dataset $\mathcal{D}$.

\paragraph{Latent Space Sampling.} The latent space generative model enables incremental extrapolation for search, and we first sample proposals at the distribution boundary to ensure a reliable shifting. Specifically, we define
\begin{align}
    y^t = y^{t-1}+\Delta_y
    \label{eq:dy}
\end{align}
where $y^{t-1}$ lies in the upper range of $\mathcal{D}^{t-1}$(e.g. the top $100$ values) and $\Delta_y$ is a fixed small increment to promote exploration beyond the current distribution. 

The proposal $\mathcal{P}^t$ can be generated by ancestral sampling,
\begin{align}
    z_0 \sim p_\theta(z_0|y) \propto p_0(z_0) p_\gamma(y | z = U_\alpha(z_0)),
\label{eq:sample_z0}
\end{align}
and then let $z = U_\alpha(z_0)$,
\begin{align}
    x\sim p(x|z= U_\alpha(z_0)),
\label{eq:sample_x}
\end{align}
where we set $y=y^t$ and $\theta=\theta^{t-1}$.
The Sampling in \cref{eq:sample_z0} can be realized by persistent Markov Chain (PMC)  by iterating~\cref{eq:Langevin},
\begin{align} 
z_0^{\tau+1} = z_0^\tau + s \nabla_{z_0} (\log p_0(z_0)+\log p_\gamma(y|U_\alpha(z_0)) + \sqrt{2s} \epsilon^\tau. 
 \label{eq:sample_pzy}
\end{align}
Here, $z_0^{\tau=0}$ is initialized from the previous training step. With PMC, it is feasible to set the number of Langevin sampling steps to be relatively small, e.g. $N=2$.
Consequently, the sampled $z$ is aware of the specific property values or constraints and regulated by the prior model. 

\begin{algorithm}[t!]
\caption{Dual-Space Optimization (DSO)}
\label{algo:dso}
\begin{algorithmic}
    \STATE {\bfseries Input:} Number of proposals~$m$, fixed increment $\Delta_y$, number of PMC steps $N$, initial parameters~$\theta_t = (\alpha_t, \beta_t, \gamma_t)$, initial dataset~$\mathcal{D}^{0}=\{z_i^0, x_i^0, y_i^0\}_{i=1}^n$, oracle function~$o(x)$, maximum shifting iteration $T$.
    \STATE {\bfseries Output:} $\theta^T$, $\mathcal{D}^T$
    \WHILE{$\E_{p_\theta(x,y)}[o(x)]$ is increasing}
    \STATE{1.\textbf{Latent space sampling}}: Sample proposal \\$\mathcal{P}^t=\{z^t_i,x^t_i, y^t_i\}_{i=1}^m$, where \\$z^t\sim p(z|y=y^{t-1}+\Delta_y)$ as in~\cref{eq:sample_z0}; \\$x^t\sim p(x|z=z^t)$ as in ~\cref{eq:sample_x}. \\
    \STATE{2.\textbf{Data space selection}}: Relabel proposal property values $y_i^t \to \check{y}_i^t=o(x_i^t)$. Update dataset \\$\mathcal{D}^{t}=\mathrm{Select}(\{z_i^t,x_i^t,\check{y}_i^t\}_{i=1}^m\cup \mathcal{D}^{t-1})$ as in~\cref{eq:select}\\
    \STATE{3.\textbf{Improve LPT}}: Learn $\theta$ using \cref{algo:learning} with $\mathcal{D}^{t}$.\\
    \ENDWHILE
\end{algorithmic}
\end{algorithm}

\paragraph{Data Space Selection.} After generating the proposals $\mathcal{P}^t$, we use the oracle function $o(x)$ to relabel these proposals, $\check{y}=o(x)$, yielding a set of generated samples and their ground-truth property values as $\{z_i^t,x_i^t,\check{y}_i^t\}_{i=1}^m$. 

The next step involves a \textit{select} operation, designed to merge these proposals with the existing dataset to improve overall properties in the new dataset. For tasks focused on optimizing properties (i.e., maximizing specific values), this is achieved by ranking all samples and retaining the top-\textit{n} entries, with \textit{n} equaling the size of dataset $\mathcal{D}^{t-1}$. Alternatively, we can also choose samples that explicitly meet certain constraints. 

The selection operation is defined as follows:
\begin{align}
    \mathcal{D}^{t}=\mathrm{Select}(\{z_i^t,x_i^t,\check{y}_i^t\}_{i=1}^m\cup \mathcal{D}^{t-1}).
    \label{eq:select}
\end{align}
This approach in the data space is a counterpart to our latent space sampling strategy. For instance, if the goal is to maximize a property $y_1$ while adhering to the constraint $y_2>c$, we would sample $z\sim p(z|y_1,y_2)\propto p(z)p(y_1|z)p(y_2|z)$ and rank the samples based on $\check{y}_1\mathds{1}(\check{y}_2>c)$, where \textit{c} is a  constant and $\mathds{1}(\cdot)$ is an indicator function.

\paragraph{Improve LPT.} 
With each generated synthetic dataset $\mathcal{D}^{t}$, we can improve the LPT using \cref{algo:learning}. The learning objective is,
\begin{align}
\theta_{t}=\arg\max_{\theta}\E_{(x,y)\sim\mathcal{D}^{t}}[\log p_{\theta}(x,y)],
\label{eq:improve}
\end{align}
where $\theta$ is initialized from $\theta^{t-1}$.

At the $t$-th shifting iteration, particularly in a single property maximization scenario, the top-$n$ selection as per \cref{eq:select} sets a threshold at $n$-th sample, denoted as $c^t$. This is because we only consider samples where $\check{y}^t=o(x^t)>c^t$. Latent space sampling and data space selection collectively result in a new dataset as a mixture of original and the synthetic data distribution.
Intuitively, training on synthetic data is a form of online learning, i.e. the samples are generated from the current model, while training on the original dataset is a form of offline learning that prevents the $\theta^t$ moving too far from the $\mathcal{D}^{t-1}$ to avoid mode collapse. 

Compared to population-based methods such as genetic algorithms~\citep{nigam2020augmenting} and particle-swarm algorithms~\citep{winter2019efficient}, our method not only maintains a shifting dataset $\mathcal{D}^t$ (which can be considered a small population), but also a shifting model $\theta^t$ to fit the dataset, so that we can improve generated molecules from the model. The model itself is virtually an infinite population because it can generate infinitely many new samples. 

Note that the \emph{select} operation in \cref{eq:select} creates a series of non-decreasing thresholds, meaning $c^t\ge c^{t-1}$. DSO terminates when there is no further increase in $c_t$, indicating that $\E_{p_\theta(x,y)}[o(x)]$ is no longer increasing.
